Instance-Sensitive Algorithms for Pure Exploration in Multinomial Logit Bandit

Motivated by real-world applications such as fast fashion retailing and online advertising, the Multinomial Logit Bandit (MNL-bandit) is a popular model in online learning and operations research, and has attracted much attention in the past decade. However, it is a bit surprising that pure exploration, a basic problem in bandit theory, has not been well studied in MNL-bandit so far. In this paper we give efficient algorithms for pure exploration in MNL-bandit. Our algorithms achieve instance-sensitive pull complexities. We also complement the upper bounds by an almost matching lower bound.

==> exp.tex <==
\section{Experiments}
\label{sec:exp}
\nicksays{add new experiments...}

We have implemented our algorithms and conducted experimental studies.  The empirical results are consistent with our theoretical predictions and have demonstrated the effectiveness of our algorithms.  We have made two main observations: (1) the $\Prune$ procedure effectively reduces the number of pulls, and (2) the improved algorithm (Algorithm~\ref{alg:improve}) outperforms the basic algorithm (Algorithm~\ref{alg:basic}), which is due to the fact that $\ExploreS$ is more effective than $\Explore$ in learning item preferences.  

\paragraph{Algorithms.} As mentioned, the algorithms proposed in this paper are the first ones for pure exploration in MNL-bandit. We name our basic algorithm (Algorithm~\ref{alg:basic}) $\Basic$, and our improved algorithm (Algorithm~\ref{alg:improve}) $\Improve$. We compare our algorithms with two baseline algorithms using the round-robin strategy.  In $\UnifB$, in each round we pull each singleton assortment once using $\Explore$ (Algorithm~\ref{alg:explore}).  In $\UnifG$, in each round we partition the $N$ items into subsets of size at most $K$ and then pull each subset once using $\ExploreS$.  Note that in all algorithms we can compute the empirical preference $\tilde{v}_i$ of any item $i$ at any time.

Our algorithms work in the fixed-confidence setting, but for the experimental study, we use the standard way to convert them into the fixed-budget setting in which the number of pulls is bounded.  The conversion is done as follows: If the number of pulls reaches the budget in the $\tau$-th round of the algorithm, then the algorithm stops making further pulls, and solves the {\em static} assortment optimization problem on the set of {\em surviving} items $I_\tau$ using their empirical preferences (in $\UnifB$ and $\UnifG$, since there is no pruning step we have $I_\tau = I$ in any round $\tau$). 

\paragraph{Datasets.} We compare the algorithms on the following synthetic and real-world datasets. 
\begin{itemize}
	\item \Unif: We set $N = 100$ and $K = 10$. The preference and reward of each item are both sampled from the uniform distribution on the interval $[0.1, 0.6]$.
	\item \Gaussian: We set $N = 100$ and $K = 10$. The preference of each item is sampled from the uniform distribution on interval $(0, 1]$, and the reward of each arm is sampled from the Gaussian distribution with mean $\mu = 0.5$ and variance $\sigma^2 = 0.01$ truncated to $(0, 1]$.
	\item \Movie: The MovieLens dataset from \cite{HK16}.\footnote{\url{https://grouplens.org/datasets/movielens/25m/}}  We select movies scored by $20,000$-$40,000$ users, and get $161$ movies. For the $i$-th movie we set $r_i$ to be the average rating divided by $5$ to obtain a value in $(0, 1]$, and $v_i$ to be the number of users that scores $i$-th movie divided by $40,000$ to obtain a value in $(0, 1]$. We set $K=10$ for the experiments.
\end{itemize} 


\begin{figure}[t]
	\begin{center}
		\includegraphics[scale=0.33]{Figs/U1.png}
		\includegraphics[scale=0.33]{Figs/U2.png}
		\includegraphics[scale=0.33]{Figs/U3.png}
	\end{center}
	\caption{Performance of algorithms for pure exploration in MNL-bandit on \Unif, \Gaussian, and \Movie\ datasets.}
	\label{fig:exp}
\end{figure}

\paragraph{Measurements.} We compare the tested algorithms by their empirical error probabilities of outputting suboptimal assortment.  All results are average of 100 runs.


\paragraph{Computational Environments.} We use programming language Kotlin to implement all algorithms. The experiments were conducted in a PowerEdge R730 server equipped with 2x Intel Xeon CPU E5-2667 v4 3.20GHz, 8-core/16-thread per CPU, and 252GB RAM.

\paragraph{Results.} Our experimental study is presented in Figure~\ref{fig:exp}.  It is easy to see that $\Improve$ achieves the best error probability.  $\Basic$ performs better than $\UnifB$, and $\Improve$ performs better than $\UnifG$.  These show that our $\Prune$ procedure (Algorithm~\ref{alg:prune}) effectively reduces the number of pulls, and consequently improves the rate of convergence to the optimal solution.

We also observe that $\UnifG$ performs better than $\UnifB$, and $\Improve$ performs better than $\Basic$.  Both phenomena are due to the fact that the $\ExploreS$ subroutine which pulls assortments with multiple items is more effective in learning item preferences than the $\Explore$ subroutine which pulls singleton assortments. This is consistent with our theoretical guarantees.

Finally, we observe that $\UnifB$ and $\Basic$ are somewhat incomparable.  On the \Unif\ and \Movie\ datasets, $\Basic$ generally performs better, while on the \Gaussian\ dataset, \Unif\  performs slightly better.  This phenomenon is due to the interplay of two forces mentioned above, that is, algorithms with $\Prune$ step is superior than those without, and subroutine $\ExploreS$ is more effective than $\Explore$.
